Towards Quantum Ray Tracing

Rendering on conventional computers is capable of generating realistic imagery, but the computational complexity of these light transport algorithms is a limiting factor of image synthesis. Quantum computers have the potential to significantly improve rendering performance through reducing the underlying complexity of the algorithms behind light transport. This paper investigates hybrid quantum-classical algorithms for ray tracing, a core component of most rendering techniques. Through a practical implementation of quantum ray tracing in a 3D environment, we show quantum approaches provide a quadratic improvement in query complexity compared to the equivalent classical approach. Based on domain specific knowledge, we then propose algorithms to significantly reduce the computation required for quantum ray tracing through exploiting image space coherence and a principled termination criteria for quantum searching. We show results for both Whitted style ray tracing, and for accelerating ray tracing operations when performing classical Monte Carlo integration for area lights and indirect illumination.

==> Approaches4QRender.tex <==
\section{Approaches for Quantum Rendering}
\label{sec:Approaches}

\begin{itemize}
    \item Make it clear that quantum is doing geometric optics
\end{itemize}

The goal of most rendering algorithms is to generate highly realistic imagery in the shortest time possible. Quantum computing provides several different routes towards this goal from both an image quality perspective, and through minimising computational time. Image quality many be able to be improved through simulating the underlying quantum mechanical nature of light transport in scenes, this is orthogonal to the approach taken in this paper which is to exploit the advantages offered by quantum algorithms to reduce the computation complexity of classical light transport algorithms.

The overall aim of these approaches is to have a fully quantum rendering system that takes a description of a scene and a camera, and allows for an image to be measured as a result. However, many significant steps from an algorithmic and hardware point of view, need to be solved before getting to that point. To this end, in this section we propose a framework which can quantify how far work is towards a full quantum rendering system.

From a starting point of a classical rendering system, the first trivial step is to employ quantum algorithms which can boost capabilities, such as true random number generation which can be easily realised from a simple quantum circuit. 

The next step towards the overall goal is to investigate entire systems which can be ported to a quantum framework. We call this "Classical with simplified quantum components". An example of this is the occlusion algorithm presented in \cite{alves2019quantum}. Due to limitations of existing quantum computers, and memory limitations for quantum simulators, these are typically restricted to highly simplified systems.

A complimentary approach is to create algorithms which can simulate more complicated effects, such as lighting, but have some of their quantum advantage removed in order to implement them on existing quantum computers or simulators. We call these methods "Classical with hybrid quantum components". Examples of this are the quantum supersampling and integration algorithms by \cite{Johnston2016} and \cite{shimada2019quantum} which demonstrate quantum advantage, yet still require classical input. The visibility algorithm in the work by \cite{alves2019quantum} also falls into this class of method due to the classical-quantum hybrid exponential search.

The next step is to have one or more components of a rendering system which are fully quantum, but work together with classical code. An example of this could be computing visibility in a complicated scene using quantum algorithms, but generating samples at each intersection using classical methods.

A final approach a a true quantum system. This would exploit quantum advantage at every stage of the rendering process, but would require significantly more resources than are available at the time of writing. This approach is discussed in the work by \cite{shimada2019quantum} who propose a full quantum system using their integration approach, but this also requires the implementation of an entire classical rendering system within the quantum computer.

%\begin{figure}[htp]
%\includegraphics{Figures/Framework.pdf}
%\end{figure}

%\begin{itemize}
%    \item Pure Quantum
%    \item Classical with Quantum components (Hybrid)
%    \item Classical with hybrid quantum components
%    \item Classical
%\end{itemize}

At each stage of this pipeline, several decisions have to be made. One primary decision is how to encode data, as quantum algorithms allow more flexibility than classical approaches. One such method is to mirror classical computing, and encode data as binary values, and then to perform operations on this binary encoded data. Another approach is to encode information into the phases or amplitudes of a register of qubits. This approach is followed in \cite{Johnston2016} to store data for supersampling.

A second decision is how to input data into the system. This is normally carried out using a series of operations to transform a system initialized in a state $|0\rangle$ into one which contains the relevant data. This naturally requires a series of gates which have to be compiled such that the required state is obtained. Another option is to use Quantum RAM \cite{giovannetti2008quantum} which could be initialised with the required state, and values read out when required.

%A third decision is what algorithms are applicable for a given problem. In Section \ref{sec:integration} we discuss multiple approaches for Monte Carlo integration; all of these can outperform classical Monte Carlo estimation in terms of oracle evaluations, but the constants in term of complexity vary significantly between algorithms.

A final decision is what is required to be measured, and how acceptable is the error. If an algorithm encodes probabilities of measuring outcomes from a given computation, there will be a probability of measuring an incorrect answer even in a simulation. A related decision is how to encode the output; if an algorithm encodes the result of a computation as the phase of a quantum register, and a resulting output is computed via the QFT, then the magnitude of the result is bounded between $[0..1]$. If values outside this range are required, a reversible encoding would be required both in the quantum algorithm and in classical post-processing.

In this paper we develop and assess the performance of quantum algorithms for ray tracing and Monte Carlo integration in simplified, but non-trivial, 3D scenes. The approaches we take are general, but due to limitations of quantum hardware at the time of writing, and the number of qubits which can be represented in a simulator, we take the route of "Classical with hybrid quantum components". This particularly impacts the ray tracing aspects, as due to limitations of the number of qubits, some computations have to be performed classically and compiled into the quantum circuit. While this allows for concrete implementations it diminishes the improvements in complexity, although as quantum hardware improves these limitations may be lifted.

%\begin{itemize}
%    \item Binary encoding
%    \item Amplitudes or Phases
%\end{itemize}

